Non-greedy Tree-based Learning for Estimating Global Optimal Dynamic Treatment Decision Rules with Continuous Treatment Dosage

Dynamic treatment regime (DTR) plays a critical role in precision medicine when assigning patient-specific treatments at multiple stages and optimizing a long term clinical outcome. However, most of existing work about DTRs have been focused on categorical treatment scenarios, instead of continuous treatment options. Also, the performances of regular black-box machine learning methods and regular tree learning methods are lack of interpretability and global optimality respectively. In this paper, we propose a non-greedy global optimization method for dose search, namely Global Optimal Dosage Tree-based learning method (GoDoTree), which combines a robust estimation of the counterfactual outcome mean with an interpretable and non-greedy decision tree for estimating the global optimal dynamic dosage treatment regime in a multiple-stage setting. GoDoTree-Learning recursively estimates how the counterfactual outcome mean depends on a continuous treatment dosage using doubly robust estimators at each stage, and optimizes the stage-specific decision tree in a non-greedy way. We conduct simulation studies to evaluate the finite sample performance of the proposed method and apply it to a real data application for optimal warfarin dose finding.

==> other.tex <==

\begin{figure}
\begin{center}
\includegraphics[width=3in]{fig1.pdf}
\end{center}
\caption{Consistency comparison in fitting surrogate model in the tidal
power example. \label{fig:first}}
\end{figure}

\begin{table}
\caption{D-optimality values for design $X$ under five different scenarios.  \label{tab:tabone}}
\begin{center}
\begin{tabular}{rrrrr}
one & two & three & four & five\\\hline
1.23 & 3.45 & 5.00 & 1.21 & 3.41 \\
1.23 & 3.45 & 5.00 & 1.21 & 3.42 \\
1.23 & 3.45 & 5.00 & 1.21 & 3.43 \\
\end{tabular}
\end{center}
\end{table}

\begin{itemize}
\item Note that figures and tables (such as Figure~\ref{fig:first} and
Table~\ref{tab:tabone}) should appear in the paper, not at the end or
in separate files.
\item In the latex source, near the top of the file the command
\verb+\newcommand{\blind}{1}+ can be used to hide the authors and
acknowledgements, producing the required blinded version.
\item Remember that in the blind version, you should not identify authors
indirectly in the text.  That is, don't say ``In Smith et. al.  (2009) we
showed that ...''.  Instead, say ``Smith et. al. (2009) showed that ...''.
\item These points are only intended to remind you of some requirements.
Please refer to the instructions for authors
at \url{http://amstat.tandfonline.com/action/authorSubmission?journalCode=uasa20&page=instructions#.VFkk7fnF_0c}
\item For more about ASA\ style, please see \url{http://journals.taylorandfrancis.com/amstat/asa-style-guide/}
\item If you have supplementary material (e.g., software, data, technical
proofs), identify them in the section below.  In early stages of the
submission process, you may be unsure what to include as supplementary
material.  Don't worry---this is something that can be worked out at later stages.
\end{itemize}
